Efficient Edge AI: Deploying Convolutional Neural Networks on FPGA with the Gemmini Accelerator

The growing concerns regarding energy consumption and privacy have prompted the development of AI solutions deployable on the edge, circumventing the substantial CO2 emissions associated with cloud servers and mitigating risks related to sharing sensitive data. But deploying Convolutional Neural Networks (CNNs) on non-off-the-shelf edge devices remains a complex and labor-intensive task. In this paper, we present and end-to-end workflow for deployment of CNNs on Field Programmable Gate Arrays (FPGAs) using the Gemmini accelerator, which we modified for efficient implementation on FPGAs. We describe how we leverage the use of open source software on each optimization step of the deployment process, the customizations we added to them and its impact on the final system's performance. We were able to achieve real-time performance by deploying a YOLOv7 model on a Xilinx ZCU102 FPGA with an energy efficiency of 36.5 GOP/s/W. Our FPGA-based solution demonstrates superior power efficiency compared with other embedded hardware devices, and even outperforms other FPGA reference implementations. Finally, we present how this kind of solution can be integrated into a wider system, by testing our proposed platform in a traffic monitoring scenario.

==> appendices.tex <==
\section{FPGA parameters}
\label{appendix:hw_details}

Tables \ref{tab:gemmini_params} and \ref{tab:vta_params} provide the configuration parameters used for the Gemmini and VTA accelerators respectively\footnote{For Gemmini, visit \url{https://github.com/ucb-bar/gemmini/blob/master/src/main/scala/gemmini/Configs.scala} for descriptions on each parameter. For VTA, visit \url{https://github.com/apache/tvm-vta/blob/main/hardware/chisel/src/main/scala/core/Configs.scala}.}. %The resource consumption of each FPGA implementation can be found on Table \ref{tab:hw_comparison}.

\begin{table}[t]
	\caption{Gemmini configuration parameters}
	\label{tab:gemmini_params}
	\begin{center}
		\begin{tabular}{cc} \toprule
			Parameter & Value \\
			\midrule
			DIM & 32 \\
			Dataflow & Weight Stationary \\
			Scratchpad capacity [KiB] & 512 \\
			Accumulator capacity [KiB] & 128 \\
			Scratchpad banks & 4 \\
			Accumulator banks & 2 \\
			Scratchpad ports & 2 \\
			Accumulator ports & 2 \\
			Input bits & 8 \\
			Accumulator bits & 32 \\
			Spatial array output bits & 18 \\
			Max in flight mem req & 32 \\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table} 

\begin{table}[t]
	\caption{VTA default configuration parameters}
	\label{tab:vta_params}
	\begin{center}
		\begin{tabular}{cc} \toprule
			Parameter & Value \\
			\midrule
			Batch size & 1 \\
			Block in size & 16 \\
			Block out size & 16 \\
			Micro-ops buffer size [KiB] & 64\\
			Input buffer size [KiB] & 16\\
			Weights buffer size [KiB] & 8\\
			Accumulator buffer size [KiB] & 64\\
			Output buffer size [KiB] & 16\\
			Input bits & 8 \\
			Weight bits & 8 \\
			Micro-ops bits & 32 \\
			Accumulator bits & 32 \\
			Output bits & 8 \\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table} 


==> optimization.tex <==
\section{Yolov7 optimizations for Gemmini deployment}
\label{section:optimizations}

	\subsection{Model related}
		
		\subsection{Sigmoid layer approximation}
			% Why do we need to approximate the sigmoid?
			% Which approximation did we used?
			% Why did we choose that approximation?
		
		
		
	\subsection{HW optimizations}
	
		% TODO: FPGA DSP packing
		
	\subsection{NN tuning}
	
		% TODO: 
